Causal Discovery Inspired Unsupervised Domain Adaptation for Emotion-Cause Pair Extraction

This paper tackles the task of emotion-cause pair extraction in the unsupervised domain adaptation setting. The problem is challenging as the distributions of the events causing emotions in target domains are dramatically different than those in source domains, despite the distributions of emotional expressions between domains are overlapped. Inspired by causal discovery, we propose a novel deep latent model in the variational autoencoder (VAE) framework, which not only captures the underlying latent structures of data but also utilizes the easily transferable knowledge of emotions as the bridge to link the distributions of events in different domains. To facilitate knowledge transfer across domains, we also propose a novel variational posterior regularization technique to disentangle the latent representations of emotions from those of events in order to mitigate the damage caused by the spurious correlations related to the events in source domains. Through extensive experiments, we demonstrate that our model outperforms the strongest baseline by approximately 11.05\% on a Chinese benchmark and 2.45\% on a English benchmark in terms of weighted-average F1 score. We have released our source code and the generated dataset publicly at: https://github.com/tk1363704/CAREL-VAE.

==> pre_experiment.tex <==
\section{Experiments}
\subsection{Experimental Setup}
\label{exp_setup}

\textbf{Datasets.} Since there is no corpus for \targettask in the UDA setting, we divide the Chinese corpus \checpe and the English corpus \enecpe into multiple domains. Since the documents in \checpe are Chinese news articles sampled from the news corpus THUCNews dataset~\cite{li2007scalable}, we employ the topic classifier THUCTC~\cite{sun2016thuctc} trained on the THUCNews dataset to categorize \checpe into 14 subsets based on topics and choose the largest five as the final domains (e.g. society, entertainment). For \enecpe, which is based on English novels, there is no high-quality classifier available. Thus we employ the topic model BERTopic~\cite{grootendorst2020bertopic} to create five topic clusters, each of them corresponds to a domain. For each corpus, we select the largest domain as the source domain, and the remaining as the target domains. The BERT embeddings of those documents for the respective corpus are visualized by t-SNE~\cite{van2008visualizing} in Figure~\ref{fig: doc_dom_visualizations}. Table~\ref{table: corpus_stat} shows the detailed statistics of each corpus.
%(e.g. society, entertainment, home, education, finance)
%In Chinese part, we adopt the THUCTC~\cite{sun2016thuctc}, a Chinese text classification toolkit developed by Tsinghua University, to divide the benchmark Chinese ECPE corpus~\cite{xia2019emotion} into various domains.
%The reason for this is that the Chinese corpus is originally constructed by taking Chinese city news from NEWS SINA\footnote{https://news.sina.com.cn/} and the THUCTC can achieve 85.6\% F1-score for text classification on the THUCNews dataset~\cite{li2007scalable}, which contains 74 million Sina news documents in 14 categories (society, entertainment, home, education, finance, etc).
%As for the English part, the benchmark English ECPE corpus~\cite{singh2021end} constructed based on English novels is selected.
%Due to the unavailability of a well-trained model for novel text classification, we separate these novels into different domains by performing topic modeling via BERTopic~\cite{grootendorst2020bertopic}, which leverages transformers~\cite{vaswani2017attention} and class-based TF-IDF~\cite{luhn1957statistical,Jones72astatistical} to create dense clusters allowing for easily interpretable topics.


\begin{figure}[hbt!]
     \centering
     \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/chi_doc_domains.png}
         \caption{Chinese}
         \label{fig: chi_docs}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/en_doc_domains.png}
         \caption{English}
         \label{fig: en_docs}
     \end{subfigure}
        \caption{The t-SNE visualizations of document embeddings in various domains for the Chinese \targettask and the English \targettask corpora.}
        \label{fig: doc_dom_visualizations}
\end{figure}


\begin{table}[hbt!]
\centering
\small
\begin{tabular}{ccc} 
\noalign{\hrule height 1.8pt}
Language                 & Domain        & \#Docs  \\ 
\hline
\multirow{5}{*}{Chinese} & Society (S)       &  1161 \\
                         & Entertainment (T) & 119     \\
                         & Home (T)          & 112     \\
                         & Education (T)     &130     \\
                         & Finance (T)       & 90      \\ 
\hline
\multirow{5}{*}{English} & History (S)   & 831 \\
                         & War (T)       & 126 \\
                         & Romance (T)   & 175 \\
                         & Adventure (T) & 127 \\
                         & Biography (T) & 95  \\
\noalign{\hrule height 1.8pt}
\end{tabular}
\caption{The statistics of the \task corpora. "S" and "T" are the abbreviations for \textit{source domain} and \textit{target domain}, respectively.}
\label{table: corpus_stat}
\end{table}


%To better meet the CD-ECPE task settings (i.e., a source domain with plenty of labeled documents while a target domain only with a small number of unlabeled ones), we respectively select 5 domains for Chinese and English.







\textbf{Metrics.} In our experiments, we use the source domain data (e.g., Society) for training and test on each target domain (e.g., Entertainment) separately.
The evaluation metrics: precision $P$, recall $R$ and F-score $F1$ for the CD-ECPE are defined as follows:

\begin{equation}
\label{eq:eval_metrics}
\begin{aligned}
& P = \dfrac{\#correctly\ predicted\ pairs}{\#predicted\ pairs}\\
& R = \dfrac{\#correctly\ predicted\ pairs}{\#ground{\text -}truth\ pairs}\\
& F1 = \dfrac{2 * P * R}{P+R}\\
\end{aligned}
\end{equation}


In addition, we also evaluate the performance on two sub-tasks including emotion clause extraction and cause clause extraction.
The corresponding evaluation metrics are same to those in Eq. \ref{eq:eval_metrics} except for substituting $pairs$ with $emotion\ clauses$ or $cause\ clauses$.


\textbf{Implementation Details.}
We adopt $\text{BERT}_{ZH}$\footnote{https://huggingface.co/hfl/chinese-roberta-wwm-ext} and $\text{BERT}_{EN}$\footnote{} as the clause and clause pair encoders for Chinese and English, respectively.
The hidden size of bidirectional LSTM for the contextual clause encoder is set to 100.
The dimensions of emotion and cause embeddings outputted by the emotion and cause encoders are set to 32.
The confidence threshold for the self-training of the emotion classifier is set to 0.6.
The number of iterations for the random-editing self-training of Vcd hierarchical neural network is set to 50.

We train the emotion classifier and Vcd hierarchical neural network using Adam optimizer, where the learning rates and the mini-batch sizes are 2e-5 and 4 and 1e-5 and 64, respectively.
As for regularization, we apply dropout to both of them with the dropout rate 0.5.







\textbf{Baselines.} To make a fair comparison, we adapt the emotion, cause and emotion-cause pair extractions of 4 existing ECPE models (i.e., Inter-EC, RankCP, MTST and UTOS) from binary classification to multi-class classification.
Besides, we integrate 3 UDA approaches on the top two best-performing ECPE models in the CD-ECPE task to further demonstrate the effectiveness of our model.
All baseline models are as follows:


\begin{figure*}[hbt!]
     \centering
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/ama_domains.png}
         \caption{Amazon sentiment reviews}
         \label{fig: amazon}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/ch_emotion.png}
         \caption{Chinese emotion clauses}
         \label{fig: chi_emotion}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/ch_cause.png}
         \caption{Chinese cause clauses}
         \label{fig: chi_cause}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/en_emotion.png}
         \caption{English emotion clauses}
         \label{fig: en_emo}
     \end{subfigure}
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/en_cause.png}
         \caption{English cause clauses}
         \label{fig: en_emo}
     \end{subfigure}
     \caption{The t-SNE visualizations of sentence embeddings for Amazon Reviews multi-domain sentiment dataset, Chinese CD-ECPE documents' emotion and cause clauses, and English CD-ECPE documents' emotion and cause clauses.}
     \label{fig:CD-ECPE_challenges}
\end{figure*}


\begin{itemize}
  \item \textbf{Inter-EC}~\cite{xia2019emotion} extracts emotion and cause clauses utilizing two hierarchical bidirectional LSTMs then pairs them and filters out the pairs that have no causality inside.
  During the emotion and cause clauses extraction, the predicted emotion clauses are used to improve cause extraction.
  
  \item \textbf{RankCP}~\cite{wei2020effective} performs the emotion-cause pair extraction using the graph attention network, which models the inter-clause information and extracts the valid emotion-cause pairs from a ranking perspective.
  
  \item \textbf{UTOS}~\cite{cheng2021unified} adopts the unified sequence labeling approach to extract emotion-cause pairs in a way that the position of emotion and cause clauses as well as how they pair can be predicted via one pass of sequence labeling.
  
  \item \textbf{MTST}~\cite{fan2021multi} solves emotion-cause pair extraction from a multi-task sequence tagging perspective, which simultaneously extracts emotion clauses and their corresponding cause clauses by using a novel distance-based tagging scheme.
  
  \item \textbf{DANN}~\cite{ganin2016domain} is an adversarial-based UDA approach that learns domain invariant representations based on the backpropagation of reverse gradients of a domain discriminator.
  
  \item \textbf{Ada-TSA}~\cite{zhang2021unsupervised} is an adapter-based UDA approach in which the newly-added adapters can capture transferable features between source and target domains by using the domain-fusion scheme.
  
  \item \textbf{MEDM}~\cite{wu2021entropy} is a minimal-entropy UDA approach that introduces diversity maximization to regulate entropy minimization for seeking a close-to-ideal domain adapotion, i.e., the minimization of source and target risks.
\end{itemize}




\subsection{Results and Analysis}
\label{sec:results}
We discuss experimental results by answering the following research questions (RQs):

\begin{table*}[hbt!]
\centering
\setlength{\tabcolsep}{4pt}
\Large
\begin{adjustbox}{width=1\textwidth}
\begin{tabular}{c|ccccccccc|ccccccccc|ccccccccc|ccccccccc}
\noalign{\hrule height 1.8pt}
\multirow{3}{*}{Model} & \multicolumn{9}{c|}{Society $\rightarrow$ Entertainment}                                              & \multicolumn{9}{c|}{Society $\rightarrow$ Home}                                              & \multicolumn{9}{c|}{Society $\rightarrow$ Education}                                               & \multicolumn{9}{c}{Society $\rightarrow$ Finance}                                               \\
                     & \multicolumn{3}{c}{EE (\%)} & \multicolumn{3}{c}{CE (\%)} & \multicolumn{3}{c|}{CD-ECPE (\%)} & \multicolumn{3}{c}{EE (\%)} & \multicolumn{3}{c}{CE (\%)} & \multicolumn{3}{c|}{CD-ECPE (\%)} & \multicolumn{3}{c}{EE (\%)} & \multicolumn{3}{c}{CE (\%)} & \multicolumn{3}{c|}{CD-ECPE (\%)} & \multicolumn{3}{c}{EE (\%)} & \multicolumn{3}{c}{CE (\%)} & \multicolumn{3}{c}{CD-ECPE (\%)}  \\
                  & $P$ & $R$ & $F1$             & $P$ & $R$ & $F1$             & $P$ & $R$ & $F1$              & $P$ & $R$ & $F1$             & $P$ & $R$ & $F1$             & $P$ & $R$ & $F1$               & $P$ & $R$ & $F1$             & $P$ & $R$ & $F1$              & $P$ & $R$ & $F1$              & $P$ & $R$ & $F1$             & $P$ & $R$ & $F1$             & $P$ & $R$ & $F1$                \\
\hline                 
\textbf{(a) Chinese}       &   &   &                &   &   &                &   &   &                  &   &   &                &   &   &                &   &   &                  &   &   &                &   &   &                 &   &   &                  &   &   &                &   &   &                &   &   &                   \\
Inter-EC    &77.39 &70.63 &73.86
            &44.90 &20.18 &27.85
            &68.42 &30.95 &42.62
            
            &75.65 &69.60 &72.50
            &54.44 &21.88 &31.21
            &63.77 &34.11 &44.44
                  
            &76.15 &72.79 &74.44
            &50.00 &13.33 &21.05
            &64.44 &21.01 &31.69
 
            &83.91 &73.74 &78.49
            &38.60 &12.64 &19.05
            &58.06 &17.65 &27.07
            \\
RankCP      &71.25 &\textbf{91.20} &80.00
            &39.29 &70.97 &50.57
            &37.72 &68.80 &48.73

            
            &79.02 &\textbf{91.13} &84.64
            &39.44 &66.14 &49.41
            &38.07 &64.84 &47.98

                  
            &79.35 &\textbf{91.11} &\textbf{84.83}
            &41.13 &69.34 &51.63
            &39.48 &67.15 &49.73

 
            &82.57 &\textbf{91.84} &\textbf{86.96}
            &44.10 &70.30 &54.20
            &43.03 &70.30 &53.38

            \\
UTOS        &\textbf{91.30} &50.40 &64.95
            &56.52 &31.45 &40.41
            &56.52 &31.20 &40.21

            &93.55 &46.77 &62.37
            &67.74 &33.60 &44.92
            &66.13 &32.03 &43.16


            &\textbf{92.96} &48.89 &64.08
            &59.15 &30.88 &40.58
            &59.15 &30.66 &40.38


            &\textbf{93.33} &42.86 &58.74
            &73.33 &33.00 &45.52
            &73.33 &32.67 &45.21


            \\
MTST        &77.88 &64.80 &70.74
            &68.75 &62.60 &65.53
            &65.18 &58.40 &61.60

            &83.70 &62.10 &71.30
            &70.00 &56.00 &62.22
            &69.00 &53.91 &60.53

                  
            &85.32 &68.89 &76.23
            &\textbf{71.19} &61.76 &66.14
            &\textbf{70.34} &60.58 &65.10

            &90.00 &64.29 &75.00
            &83.56 &60.40 &70.11
            &78.08 &56.44 &65.52

            \\
Ours        &85.22 &77.78 &\textbf{81.33}
            &\textbf{78.12} &\textbf{78.74} &\textbf{78.43}
            &\textbf{78.12} &\textbf{78.74} &\textbf{78.43}

            &\textbf{94.34} &80.00 &\textbf{86.58}
            &\textbf{84.30} &\textbf{77.86} &\textbf{80.95}
            &\textbf{84.30} &\textbf{77.86} &\textbf{80.95}
                  
            &78.17 &81.62 &79.86
            &69.14 &\textbf{80.58} &\textbf{74.42}
            &69.14 &\textbf{80.58} &\textbf{74.42}
 
            &89.01 &81.82 &85.26
            &\textbf{96.39} &\textbf{78.43} &\textbf{86.49}
            &\textbf{96.39} &\textbf{78.43} &\textbf{86.49}
            \\
\hline
\textbf{(b) English}       & \multicolumn{9}{c|}{History $\rightarrow$ War}                                              & \multicolumn{9}{c|}{History $\rightarrow$ Romance}                                      & \multicolumn{9}{c|}{History $\rightarrow$ Adventure        }                                       & \multicolumn{9}{c}{History $\rightarrow$ Biography}                                               \\
Inter-EC          &51.97 &31.73 &39.40
                  &26.92 &14.06 &18.47
                  &46.55 &12.74 &20.00
 
                  
                  &54.17 &37.57 &44.37
                  &32.76 &12.58 &18.18
                  &53.97 &16.04 &24.73

                  
                  &48.73 &44.51 &46.53
                  &27.40 &15.04 &19.42
                  &48.08 &23.70 &31.75

                  
                  &59.74 &47.92 &53.18
                  &21.23 &11.65 &15.05
                  &51.35 &17.92 &26.57
                  \\
RankCP            &43.86 &55.56 &49.02
                  &38.98 &52.27 &44.66
                  &31.67 &42.22 &36.19

                  &43.24 &56.14 &48.85
                  &35.71 &48.39 &41.10
                  &26.37 &38.71 &31.37

                  &56.10 &\textbf{66.67} &60.93
                  &30.51 &40.45 &34.78
                  &25.40 &35.56 &29.63

                  &52.94 &58.06 &55.38
                  &29.31 &50.00 &36.96
                  &23.73 &41.18 &30.11

                  
                  \\
UTOS              &\textbf{87.50} &22.40 &35.67
                  &75.00 &19.35 &30.77
                  &75.00 &19.20 &30.57

                  &\textbf{87.88} &23.39 &36.94
                  &\textbf{81.82} &21.60 &34.18
                  &\textbf{78.79} &20.31 &32.30


                  &\textbf{87.10} &20.00 &32.53
                  &\textbf{83.87} &19.12 &31.14
                  &77.42 &17.52 &28.57


                  &\textbf{90.91} &20.41 &33.33
                  &72.73 &16.00 &26.23
                  &72.73 &15.84 &26.02

                  \\
MTST              &53.16 &\textbf{74.81} &\textbf{62.15}
                  &41.15 &\textbf{68.38} &51.38
                  &32.74 &54.01 &40.77

                  
                  &53.80 &\textbf{68.55} &\textbf{60.28}
                  &45.31 &\textbf{69.60} &54.89
                  &31.77 &47.66 &38.13

                  
                  &62.04 &54.03 &57.76
                  &37.14 &52.00 &43.33
                  &29.71 &40.62 &34.32

                  
                  &56.10 &\textbf{68.15} &\textbf{61.54}
                  &46.20 &62.50 &53.13
                  &33.70 &45.26 &38.63

 
                  
                  \\
Ours              &63.55 &53.54 &58.12
                  &\textbf{86.67} &59.54 &\textbf{70.59}
                  &\textbf{86.67} &\textbf{59.54} &\textbf{70.59}
                  
                  &60.00 &50.00 &54.55
                  &59.52 &52.91 &\textbf{56.02}
                  &59.52 &\textbf{52.91} &\textbf{56.02}
                  
                  &67.24 &60.47 &\textbf{63.67}
                  &78.15 &\textbf{64.14} &\textbf{70.45}
                  &\textbf{78.15} &\textbf{64.14} &\textbf{70.45}
                  
                  &51.09 &48.96 &50.00
                  &\textbf{91.46} &\textbf{75.00} &\textbf{82.42}
                  &\textbf{91.46} &\textbf{75.00} &\textbf{82.42}
                  \\
\noalign{\hrule height 1.8pt}
\end{tabular}
\end{adjustbox}
\caption{Experimental results of our models and baseline models utilizing precision (P), recall (R), and F1 score (F1) as metrics on the CD-ECPE task. EE, CE and CD-ECPE denote Emotion Extraction, Cause Extraction and Cross-Domain Emotion-Cause Pair Extraction respectively.}
\label{table: exp_results}
\end{table*}

\textbf{RQ1:  What are the special challenges for emotion-cause pair extraction in the UDA setting?}
To have an intuitive understanding of the challenges of the CD-ECPE task, we visualize the sentence embeddings for a representative UDA benchmark dataset Amazon Reviews~\cite{blitzer2007biographies} and our bilingual CD-ECPE dataset using t-SNE.
As shown in Figure~\ref{fig:CD-ECPE_challenges}, the spatial distribution of different domains in Amazon Reviews is not quite different and even overlapping, thus this can be effortlessly solved by utilizing conventional UDA approaches like common shared feature learning.
As for the bilingual CD-ECPE dataset, the distribution of emotions in various domains has no discriminative structure while the distribution of causes shows an obvious cluster structure and each cluster is far away from the other.
Such the circumstance makes existing UDA approaches may not be applicable as they are only workable when the distribution shift from a source domain to a target domain is small, i.e., two domains are not too far~\cite{zhao2019learning,kumar2020understanding}.


\begin{table*}[hbt!]
\centering
\setlength{\tabcolsep}{4pt}
\Large
\begin{adjustbox}{width=1\textwidth}
\begin{tabular}{c|ccccccccc|ccccccccc|ccccccccc|ccccccccc}
\noalign{\hrule height 1.8pt}
\multirow{3}{*}{Model} & \multicolumn{9}{c|}{Society $\rightarrow$ Entertainment}                                              & \multicolumn{9}{c|}{Society $\rightarrow$ Home}                                              & \multicolumn{9}{c|}{Society $\rightarrow$ Education}                                               & \multicolumn{9}{c}{Society $\rightarrow$ Finance}                                               \\
                   & \multicolumn{3}{c}{EE (\%)} & \multicolumn{3}{c}{CE (\%)} & \multicolumn{3}{c|}{CD-ECPE (\%)} & \multicolumn{3}{c}{EE (\%)} & \multicolumn{3}{c}{CE (\%)} & \multicolumn{3}{c|}{CD-ECPE (\%)} & \multicolumn{3}{c}{EE (\%)} & \multicolumn{3}{c}{CE (\%)} & \multicolumn{3}{c|}{CD-ECPE (\%)} & \multicolumn{3}{c}{EE (\%)} & \multicolumn{3}{c}{CE (\%)} & \multicolumn{3}{c}{CD-ECPE (\%)}  \\
                  & $P$ & $R$ & $F1$             & $P$ & $R$ & $F1$             & $P$ & $R$ & $F1$              & $P$ & $R$ & $F1$             & $P$ & $R$ & $F1$             & $P$ & $R$ & $F1$               & $P$ & $R$ & $F1$             & $P$ & $R$ & $F1$              & $P$ & $R$ & $F1$              & $P$ & $R$ & $F1$             & $P$ & $R$ & $F1$             & $P$ & $R$ & $F1$                \\
\hline                 
\textbf{(a) Chinese}       &   &   &                &   &   &                &   &   &                  &   &   &                &   &   &                &   &   &                  &   &   &                &   &   &                 &   &   &                  &   &   &                &   &   &                &   &   &                   \\
RankCP+Ada-TSA    &82.24 &89.80 &85.85
                  &38.83 &72.28 &50.52
                  &37.70 &71.29 &49.32
                  
                  &78.95 &91.84 &84.91
                  &41.62 &71.29 &52.55
                  &39.66 &70.30 &50.71
                  
                  &75.65 &88.78 &81.69
                  &44.20 &60.40 &51.05
                  &41.13 &57.43 &47.93

                  
                  &84.62 &89.80 &87.13
                  &43.35 &74.26 &54.74
                  &41.57 &73.27 &53.05

            \\
RankCP+DANN      &85.29 &92.80 &88.89
                 &44.84 &80.65 &57.64
                 &44.05 &80.00 &56.82

                 &87.12 &\textbf{92.74} &\textbf{89.84}
                 &46.67 &\textbf{82.68} &59.66
                 &45.33 &\textbf{79.69} &57.79

                 &82.89 &\textbf{93.33} &87.80
                 &42.63 &78.10 &55.15
                 &40.86 &76.64 &53.30

                 &84.76 &\textbf{90.82} &\textbf{87.68}
                 &48.81 &\textbf{81.19} &60.97
                 &46.51 &\textbf{79.21} &58.61


            \\
RankCP+MEDM       &\textbf{87.62} &\textbf{93.88} &\textbf{90.64}
                  &45.36 &\textbf{82.18} &58.45
                  &44.86 &\textbf{82.18} &58.04

                  &84.83 &91.11 &87.86
                  &54.74 &75.91 &63.61
                  &52.04 &74.45 &61.26
                  
                  &\textbf{85.71} &91.84 &\textbf{88.67}
                  &49.11 &\textbf{82.18} &61.48
                  &47.40 &\textbf{81.19} &59.85

                  
                  &86.61 &88.71 &87.65
                  &62.24 &70.08 &65.93
                  &59.06 &68.75 &63.54


            \\
MTST+Ada-TSA      &82.73 &72.80 &77.45
                  &66.67 &68.29 &67.47
                  &63.49 &64.00 &63.75

                  
                  &89.19 &79.84 &84.26
                  &71.54 &70.40 &70.97
                  &69.92 &67.19 &68.53

                  
                  &77.70 &80.00 &78.83
                  &60.90 &69.85 &65.07
                  &56.41 &64.23 &60.07

                  
                  &88.37 &77.55 &82.61
                  &65.62 &62.38 &63.96
                  &64.58 &61.39 &62.94


            \\
MTST+DANN        &80.18 &71.20 &75.42
                 &64.75 &64.23 &64.49
                 &63.93 &62.40 &63.16

                  
                  &87.23 &66.13 &75.23
                  &70.00 &56.00 &62.22
                  &67.00 &52.34 &58.77
                  
                  &75.81 &69.63 &72.59
                  &\textbf{69.53} &65.44 &67.42
                  &64.06 &59.85 &61.89
                  
                  &88.16 &68.37 &77.01
                  &76.25 &60.40 &67.40
                  &71.25 &56.44 &62.98


            \\
MTST+MEDM        &85.58 &71.20 &77.73
                 &73.58 &63.41 &68.12
                 &73.58 &62.40 &67.53
                  
                 &63.91 &68.00 &65.89
                 &63.70 &69.92 &66.67
                 &57.04 &61.60 &59.23

                 &71.88 &68.15 &69.96
                 &65.94 &66.91 &66.42
                 &60.14 &60.58 &60.36
                  
                 &78.91 &81.45 &80.16
                 &65.19 &70.40 &67.69
                 &63.70 &67.19 &65.40


            \\
Ours        &85.22 &77.78 &81.33
            &\textbf{78.12} &78.74 &\textbf{78.43}
            &\textbf{78.12} &78.74 &\textbf{78.43}

            &\textbf{94.34} &80.00 &86.58
            &\textbf{84.30} &77.86 &\textbf{80.95}
            &\textbf{84.30} &77.86 &\textbf{80.95}
                  
            &78.17 &81.62 &79.86
            &69.14 &80.58 &\textbf{74.42}
            &\textbf{69.14} &80.58 &\textbf{74.42}
 
            &\textbf{89.01} &81.82 &85.26
            &\textbf{96.39} &78.43 &\textbf{86.49}
            &\textbf{96.39} &78.43 &\textbf{86.49}
            \\
\hline
\textbf{(b) English}       & \multicolumn{9}{c|}{History $\rightarrow$ War}                                              & \multicolumn{9}{c|}{History $\rightarrow$ Romance}                                      & \multicolumn{9}{c|}{History $\rightarrow$ Adventure        }                                       & \multicolumn{9}{c}{History $\rightarrow$ Biography}                                               \\
RankCP+Ada-TSA    &44.23 &51.11 &47.42
                  &41.27 &59.09 &48.60
                  &30.88 &46.67 &37.17

                  
                  &50.70 &63.16 &56.25
                  &28.57 &41.94 &33.99
                  &27.47 &40.32 &32.68

                  
                  &48.10 &55.07 &51.35
                  &40.00 &49.44 &44.22
                  &29.31 &37.78 &33.01

                  
                  &44.44 &51.61 &47.76
                  &31.25 &44.12 &36.59
                  &26.00 &38.24 &30.95

            \\
RankCP+DANN      &50.88 &64.44 &56.86
                 &46.77 &\textbf{65.91} &54.72
                 &36.62 &57.78 &44.83

                  
                 &56.92 &64.91 &60.66
                 &35.05 &54.84 &42.77
                 &29.41 &48.39 &36.59
                  
                 &58.11 &62.32 &60.14
                 &35.59 &47.19 &40.58
                 &31.15 &42.22 &35.85
                  
                 &58.82 &64.52 &61.54
                 &43.18 &55.88 &48.72
                 &27.66 &38.24 &32.10


            \\
RankCP+MEDM        &57.69 &66.67 &61.86
                  &45.76 &61.36 &52.43
                  &39.39 &57.78 &46.85

                  
                  &\textbf{66.67} &70.18 &\textbf{68.38}
                  &34.62 &58.06 &43.37
                  &31.13 &53.23 &39.29

                  
                  &55.70 &\textbf{63.77} &59.46
                  &37.50 &50.56 &43.06
                  &33.06 &45.56 &38.32
                  
                  &63.89 &\textbf{74.19} &\textbf{68.66}
                  &36.21 &61.76 &45.65
                  &26.98 &50.00 &35.05


            \\
MTST+Ada-TSA      &59.67 &80.00 &68.35
                  &41.38 &61.76 &49.56
                  &37.44 &55.47 &44.71

                  
                  &56.29 &69.63 &62.25
                  &44.89 &58.09 &50.64
                  &39.20 &50.36 &44.09

                  
                  &59.26 &47.41 &52.67
                  &31.03 &39.71 &34.84
                  &27.01 &34.31 &30.23

                  
                  &62.42 &72.59 &67.12
                  &45.56 &56.62 &50.49
                  &41.42 &51.09 &45.75


            \\
MTST+DANN         &62.35 &78.52 &69.51
                  &43.78 &59.56 &50.47
                  &39.46 &53.28 &45.34

                  
                  &57.71 &\textbf{74.81} &65.16
                  &45.26 &63.24 &52.76
                  &40.00 &\textbf{55.47} &46.48

                  
                  &59.32 &56.00 &57.61
                  &31.61 &49.59 &38.61
                  &25.91 &40.00 &31.45

                  
                  &\textbf{63.91} &62.96 &63.43
                  &53.69 &58.82 &56.14
                  &46.98 &51.09 &48.95


            \\
MTST+MEDM         &\textbf{68.45} &\textbf{85.19} &\textbf{75.91}
                  &41.88 &58.82 &48.93
                  &39.27 &54.74 &45.73

                  
                  &52.00 &62.40 &56.73
                  &50.97 &\textbf{64.23} &\textbf{56.83}
                  &44.52 &55.20 &49.29

                  
                  &\textbf{69.09} &60.80 &\textbf{64.68}
                  &29.13 &54.47 &37.96
                  &26.09 &48.00 &33.80

                  
                  &53.99 &65.19 &59.06
                  &50.88 &63.97 &56.68
                  &41.52 &51.82 &46.10

            \\
Ours              &63.55 &53.54 &58.12
                  &\textbf{86.67} &59.54 &\textbf{70.59}
                  &\textbf{86.67} &\textbf{59.54} &\textbf{70.59}
                  
                  &60.00 &50.00 &54.55
                  &\textbf{59.52} &52.91 &56.02
                  &\textbf{59.52} &52.91 &\textbf{56.02}
                  
                  &67.24 &60.47 &63.67
                  &\textbf{78.15} &\textbf{64.14} &\textbf{70.45}
                  &\textbf{78.15} &\textbf{64.14} &\textbf{70.45}
                  
                  &51.09 &48.96 &50.00
                  &\textbf{91.46} &\textbf{75.00} &\textbf{82.42}
                  &\textbf{91.46} &\textbf{75.00} &\textbf{82.42}
                  \\
\noalign{\hrule height 1.8pt}
\end{tabular}
\end{adjustbox}
\caption{Experimental results of our models and the UDA variants of the top two best-performing baseline models on the CD-ECPE task. All metrics are the same as those in Table \ref{table: exp_results}.}
\label{table: exp_results_uda}
\end{table*}

\textbf{RQ2: Why are the proposed models able to outperform the baseline models in new domains?}
Table~\ref{table: exp_results} reports the comparative results of our models and the baseline models on the CD-ECPE task as well as two sub-tasks, i.e., emotion extraction (EE) and cause extraction (CE).
Our models outperform all baseline models for both CE and CD-ECPE, which obtain $14.07\%$ (CE), $16.88\%$ (CD-ECPE) and $19.19\%$ (CE), $31.91\%$ (CD-ECPE) $F1$ improvements on average for Chinese and English over the best-performing baseline model MTST.
Specifically, such the advantage is principally rooted in the significant improvement of CE as we can see the performance of our models in EE is not always superior to other baseline models (e.g., RankCP for Chinese and MTST for English).
This observation suggests that, causal discovery enables our model to learn the underlying causal mechanism between emotion and cause and leverage the learned causal knowledge when adapting to a new domain.

Besides, we also investigate the possible reasons for the unsatisfactory results produced by the baseline models.
Regarding the two-step pipeline model, Inter-EC adopts two individual models for EE and CE and uses the emotion predictions to enhance the cause predictions then pairs them, however, the correlations between emotions and causes are different in various domains as their emotion distributions are similar while cause distributions are diverse, therefore leading to the good performance on EE but not on CE as well as CD-ECPE.
RankCP employs inter-clause modeling enhanced with a kernel-based relative position scheme to extract emotion-cause pairs, which has a similar problem as Inter-EC because the interrelations between emotions and causes are varying from domain to domain.
Although the inter-clause modeling suffers from domain shift, the relative position scheme is still helpful for CE and CD-ECPE based on the cohesion and coherence of discourse~\cite{de1981introduction}, i.e., the distance between emotion and cause clauses in different domains may be relatively similar.
UTOS performs the emotion-cause pair extraction through a unified sequence labeling that sequentially predicts the label of each clause in a document.
Such the manner still implicitly exploits the relevance between emotions and causes and therefore has the similar performance as Inter-EC.
MTST emphasizes on explicitly modeling the correlations and information interaction between emotions and causes, in which the relative distances between emotion and causes predictions are directly used to refined the predictions of emotion-cause pairs.
This results in the relative good performance on EE, CE and CD-ECPE compared to other baseline models.




\textbf{RQ3: What are the difficulties of cause extraction and the importance of utilizing the dependence between emotions and causes? To answer this question, we compare our approach with the SOTA UDA approaches.}

Table \ref{table: exp_results_uda} reports comparative results of
our models and the UDA variants (Ada-TS, DANN and MEDM mentioned in Section \ref{exp_setup}) of the top two best-performing baseline models (RankCP and MTST) on the CD-ECPE task.
It can be observed that MEDM is superior to
the other two UDA approaches based on the average CD-ECPE $F1$ for different target domains in Chinese and English., indicating that the trade-off between entropy minimization and prediction diversity is indeed useful for UDA.
However, it still falls short of CE in UDA setting as the improvements of CD-ECPE $F1$ are mainly attribute to EE (e.g., MTST-MEDM has an average of $3.67\% $ EE and $-0.58\%$ CE $F1$ improvements compared to MTST in English).
Regarding DANN and Ada-TS, both cannot learn the domain-invariant  emotion features without compromising the domain-specific cause features, resulting in inferior performance to MEDM.

In comparison with all UDA variant baseline models, our models consistently outperform them on both CE and CD-ECPE according to the corresponding $F1$s regardless of Chinese and English.
In addition, although our models only achieve comparable performance to most UDA variants on EE, they still achieve significantly superior CE $F1$.
This clearly demonstrates the importance of utilizing causal discovery to identify the dependence between emotions and causes after causal disentanglement.

\textbf{RQ4: How do different constraints/regularizations influence the model performance?}

To investigate the influences of different regularizations, we select two independence measures Hilbert–Schmidt independence criterion~\cite[(HSIC]{gretton2005measuring} and Variation of Information~\cite[(VI]{cheng2020improving} that are commonly used for disentangled representation
learning to replace the MMD loss, the results on Chinese CD-ECPE task are given in Table \ref{table: exp_results_regularization} due to page limit.
Observe that using HSIC and VI lead to performance degradation.
This indicates that enforcing the independence between emotions and causes hurts the learning of emotion and cause random variables as they are causally related, and eventually affects the performance of causal discovery.
On the other hand, such results verify that the MMD loss is crucial for approximating random variables with causal relations. 

\begin{table}[hbt!]
\centering
\Large
\begin{adjustbox}{width=1\linewidth}
\begin{tabular}{c|ccc|ccc|ccc|ccc}
\noalign{\hrule height 1.8pt}
\multirow{3}{*}{Model} & \multicolumn{3}{c|}{Society $\rightarrow$ Entertainment}                                              & \multicolumn{3}{c|}{Society $\rightarrow$ Home}                                              & \multicolumn{3}{c|}{Society $\rightarrow$ Education}                                               & \multicolumn{3}{c}{Society $\rightarrow$ Finance}                                               \\
                  & \multicolumn{3}{c|}{CE \& CD-ECPE (\%)} &  \multicolumn{3}{c|}{CE \& CD-ECPE (\%)} &  \multicolumn{3}{c|}{CE \& CD-ECPE (\%)} &  \multicolumn{3}{c}{CE \& CD-ECPE (\%)}  \\
                 & $P$ & $R$ & $F1$               & $P$ & $R$ & $F1$             & $P$ & $R$ & $F1$              & $P$ & $R$ & $F1$                                                     \\
\hline                 
HSIC        &59.87 &73.23 &65.88
           
            
            &60.51 &71.76 &65.66
            
                  
            &61.73 &73.38 &67.05
            
 
            &74.23 &71.57 &72.88
            \\
VI          &63.51 &74.02 &68.36
           
            
            &65.97 &72.52 &69.09
            
                  
            &60.24 &71.94 &65.57
            
 
            &79.12 &70.59 &74.61

            \\
bh goal1    &61.66 &61.42 &61.54
           
            
            &59.50 &75.57 &66.58
            
                  
            &62.91 &76.26 &68.94
            
 
            &70.31 &77.45 &73.71

            \\
bh goal2    &76.52 &79.53 &77.99
           
            
            &74.80 &72.52 &73.64
            
                  
            &76.35 &81.29 &78.75
            
 
            &93.10 &79.41 &85.71
            \\
MMD         
            &\textbf{78.12} &\textbf{78.74} &\textbf{78.43}

            
            &\textbf{84.30} &\textbf{77.86} &\textbf{80.95}
                  
            
            &\textbf{69.14} &\textbf{80.58} &\textbf{74.42}
 
            
            &\textbf{96.39} &\textbf{78.43} &\textbf{86.49}
            \\
\noalign{\hrule height 1.8pt}
\end{tabular}
\end{adjustbox}
\caption{Experimental results of our models with different regularizations on Chinese CD-ECPE task. Since EE for all regularizations are the same, we omit them and only report CE and CD-ECPE. These two metrics are the same as those in Table \ref{table: exp_results}.}
\label{table: exp_results_regularization}
\end{table}

\textbf{RQ5: How does disentangled representation learning improve model performance, in which cases?}

To study the effect of disentangled representation learning, we remove the MMD loss during model training as it is the key for disentanglement, the experimental results of this variant model and our original model are shown in Figure \ref{fig:wommd_mmd_results}.
As observed, our original model can achieve better performance compared to its variant, demonstrating that disentangled representation learning can boost the CD-ECPE performance.

\begin{figure}[hbt!]
\centering
\includegraphics[width=\linewidth]{figures/wo_mmd.png}
\caption{Experimental results of our variant models that remove the MMD loss (denoted as "CDDUDA w/o MMD") and our original models CDDUDA.}
\label{fig:wommd_mmd_results}
\end{figure}

To further understand how the MMD loss contributes to the CD-ECPE, we examine the performance of our original model and its variant for two different types of emotion-cause pairs including normal and self-chain, the results are shown in Figure \ref{fig:normal_self_results}.
Observe that the performance improvement is mainly attributed to the significant increment of precision in self-chain cases.
This suggests that disentangled representation learning helps approximate emotion and cause random variables from emotion-cause pairs, and ultimately aids in the causal discovery process.


\begin{figure}[hbt!]
\centering
\includegraphics[width=\linewidth]{figures/normal_self.png}
\caption{Experimental results of CDDUDA w/o MMD and CDDUDA for normal and self-chain cases. The normal case refers to an emotion-cause pair composed of two different clauses, while the self-chain case is composed of the same clause.}
\label{fig:normal_self_results}
\end{figure}


\textbf{RQ6: Is there a risk that the model memorises the examples in the target domain during self-training? If not, why?}

\begin{figure}[hbt!]
\centering
\includegraphics[width=\linewidth]{figures/self_train_random_editting_analysis.png}
\caption{Experimental results of our variant models that fixes negative samples during the self-training (denoted as "CDDUDA w/ FN") and our original models CDDUDA.}
\label{fig:self_train_random_editting_analysis}
\end{figure}



Report the proportion of changed positive examples and the proportion of changed examples in each iteration. Validation/test set performance in each iteration.
precision/recall/F1 changes over the time.

1. If the negative examples do not change over the time.
2. If the model is not pretrained in the source domain.
















==> pre_meth.tex <==
\section{Methodology}
In this section, we start with the task definition of cross-domain emotion-cause pair extraction.
Then, we provide an overview of our proposed approach named  Causal Disentanglement-Discovery Unsupervised Domain Adaptation (CDDUDA).
Finally, we elaborate on the CDDUDA based on the aforementioned preliminary knowledge.

\begin{figure*}[hbt!]
\centering
\includegraphics[width=\linewidth]{figures/mod_overview.png}
\caption{Overview of Causal Disentanglement-Discovery Unsupervised Domain Adaptation (CDDUDA).}
\label{fig:mod_overview}
\end{figure*}



\subsection{Task Definition}
A formal definition of the cross-domain emotion-cause pair extraction (CD-ECPE) task is as follows: 
Given a source domain $D^s = \{(d^{s}_{1}, P^{s}_{1}), (d^{s}_{2}, P^{s}_{2}), ..., (d^{s}_{n}, P^{s}_{n}) \}$ consisting of $N^s$ labeled documents, and a target domain $D^t = \{(d^{t}_{1}, ?), (d^{t}_{2}, ?), ..., (d^{t}_{n}, ?) \}$ consisting of $N^t$ unlabeled documents. 
Each document contains multiple clauses $d=(c_1,c_2, ..., c_{|d|})$ and a set of emotion-cause pairs $P=\{(c^{e_1}, c^{c_1}), (c^{e_2}, c^{c_2}), ..., (c^{e_n}, c^{c_n})\}$ (the pairs are unknown in the target domain), where $c^{e_n}$ is an emotion clause and $c^{c_n}$ is the corresponding cause clause.
The goal of CD-ECPE is to train an effective classifier that can adapt from a source domain to a target domain, thereby extracting the emotion-cause pairs of unlabeled documents in the target domain.
Note that the CD-ECPE task is defined at the clause level as depicting emotion causes at the word or phrase level is arduous.

In the original emotion-cause pair extraction (ECPE) task~\cite{xia2019emotion}, it assumes training and test documents are independently and identically distributed (i.i.d.) samples drawn from a distribution, which is often not valid in practice due to potential distribution shift.
In comparison, the CD-ECPE task is more realistic and difficult as it allows documents to span various domains in which their distributions are different and requires a model can transfer the knowledge from label rich domain (source domain) to the label none domain (target domain).



\subsection{CDUDA Overview}
In CD-ECPE, we aim to identify the emotion-cause pairs in the target domain by drawing on the source domain causal knowledge.
Nevertheless, transferring such knowledge is difficult as the emotions between the source and target domains are usually similar but the causes are variant.
For instance, in society (source) and finance (target) domains, the same emotion clause "I feel so happy today" can be caused by two different cause clauses "I receive a grant from the government" and "The stock I bought went up", respectively. 
This makes common UDA approaches (e.g., common shared feature learning, domain adversary and pre-training) may not be applicable due to the difficulty of learning causally related domain-invariant (emotion) and domain-specific (cause) representations in parallel.

To address this challenge, we consider tackling the CD-ECPE task from the perspective of causal discovery rather than standard UDA.
Specifically, if we are able to discover the high-level causal variables regarding emotions and causes (i.e., identify the causal relations between random variables that represent emotions and causes) in a source domain, then it is easy to transfer such causal knowledge from the source domain to a target domain as the underlying causal mechanism between emotions and causes remains unchanged across different domains.
% \tw{a little bit too abstract here. Is it possible to show an example here?}
For instance, all the specific causes of emotion "happy" can be viewed as the values of a random variable $C_{happy}$, similarly, $E_{happy}$ is another random variable that concludes all possible emotion values.
Although the specific causes (i.e., the values of $C_{happy}$) of various domains are different, the causal relation $C_{happy} \rightarrow E_{happy}$ remain the same, that is, the discovery of causal variables makes the cross-domain (causal) knowledge transfer considerably easier.
Once the causal variables regarding emotions and causes in the target domain are discovered through knowledge transfer,  the corresponding emotion-cause pairs can be naturally derived \tw{This paragraph is key but starting from ``that is, the discovery of causal variables makes the cross-domain....'' is not clear enough yet I think. Starting from here, we need to point it out explicitly what is the thing we can transfer and how this transferred thing can help with the task on the target domain}.


To discover causal variables in a source domain, we need to obtain a set of random variables representing emotions and causes and then identify the causal relations between them.
Obviously, these (causal) random variables are not independent but causally related, we thus consider using causal disentanglement and discovery simultaneously to obtain them.
As shown in Figure~\ref{fig:mod_overview} Step 2, it is a VAE-based model containing two parts: (1) clause pair, emotion and cause encoders, emotion and cause classifiers, and a clause pair decoder are responsible for causal disentanglement. (2) a pair classifier is responsible for causal discovery.

In the (1), the entangled representations of emotions and causes produced by the clause pair encoder are passed to the emotion and cause encoders, which first encode them to emotion and cause latent spaces then map such latent spaces' emotion and cause expressions to corresponding distributions.
This mapping is consistent with the definition of random variable~\cite{papoulis2002probability}. \tw{I think an explicit mention of the definition of random variable would be helpful here}
Thus, the learning of mapping functions can be considered as the acquisition of random variables.
To ensure the obtained random variables preserve causal relations and emotion and cause information \tw{a little bit unclear here. random variables can preserve causal relations?}, we leverage maximum mean discrepancy (MMD)~\cite{gretton2012kernel} to separate the emotion and cause random variables (i.e., the emotion and cause random variables' distributions are different but can be dependent), and labels of emotions and causes to guarantee the samples of such variables are discriminative for emotions and causes (i.e., provide sufficient information for the emotion and cause classifiers for prediction).
On top of these, the clause pair decoder ensures the samples of separated emotion and cause random variables are able to reconstruct originally inputted emotion-cause pairs.

For the (2), the pair classifier is used to determine whether the samples of separated emotion and cause random variables are dependent, and then infer the causal relations between these random variables.
The reason for this is that the edge direction is naturally pointed from a cause to an emotion in causal discovery, once the dependence between them is determined (i.e., a edge exists), the causal relation can be discovered. 
By training these two parts jointly, we can discover the source domain's causal variables in an efficient way.

To enable cross-domain causal knowledge transfer, we consider using a self-training approach to achieve it.
However, given a set of documents in a target domain, for each document, we have to pair each clause individually with the remaining clauses to construct all possible pairs based on the aforementioned causal variables discovering process, which makes the transfer learning clumsy as not each clause contains an emotion or a cause.
To ease the transfer learning process, we exploit the nature of emotion (i.e., emotions are similar across various domains) to first extract emotions in a target domain using self-training~\cite{chen2011co}, as shown in Figure~\ref{fig:mod_overview} Step 1.
Subsequently, we construct all possible pairs for each target domain document only based on its extracted emotion clause(s).

To put Step 1 and 2 together, CDDUDA first performs emotion extraction on the target domain documents using self-training~\cite{chen2011co} based on the knowledge learned from the source domain.
After obtaining the emotions, CDDUDA simultaneously extracts the causes and emotion-cause pairs of target domain documents in a way of causal disentanglement and discovery through random-editing self-training (introduced in Section \ref{section:cau_par_extraction}).

% This is achieved by leveraging maximum mean discrepancy (MMD)~\cite{gretton2012kernel} and labels of emotions and causes within the framework of VAE, as shown in Figure~\ref{fig:mod_overview} Step 2.


% The reason for adopting MMD and labels of emotions and causes is that the former ensures the emotion and cause random variables are different but causally related by maximizing the MMD between their distributions, while the latter ensures such variables contain the emotion and cause information by using their values for emotion and cause predictions.






% In causal discovery, the emotions and causes can be treated as the samples of a set of random variables, our goal is now to infer the causal graphs (i.e., edges with directions) from such variables in the target domain by taking advantage of the knowledge from the source domain.
% That is, given an emotion random variable $E$ and a cause random variable $C$, we intend to conclude whether $ C \rightarrow E$ ($C$ causes $E$) but not the opposite as the edge directions are naturally pointed from the cause to the emotion.



% To obtain emotion and cause random variables without losing the causal relations between them, we adopt VAE to achieve 






% using causal disentanglement to obtain causal disentangled representations $E^{t}=\{E^{t}_{1}, E^{t}_{2}, ..., E^{t}_{n}\}$ and $C^{t}=\{C^{t}_{1}, C^{t}_{2}, ..., C^{t}_{n}\}$ for emotions and causes in the target domain 
% Then, we treat these representations as a set of random variables that enable us to perform causal discovery to identify the causal relations (i.e., emotion-cause pairs). between them.
% That is, given the sample $\mathcal{D}=\{(e^{t}_{1}, c^{t}_{1}), (e^{t}_{2}, c^{t}_{2}), ..., (e^{t}_{n}, c^{t}_{n})\} \sim P(E_{i}, C_{j})$, for a Cartesian product of $E^{t}$ and $C^{t}$, our goal is to infer the causal graphs $\mathcal{G}=\{\mathcal{G}_{1}, \mathcal{G}_{2}, ..., \mathcal{G}_{n}\}$ that conclude whether $ C_{j} \rightarrow E_{i}$ but not the opposite as the edge directions are naturally pointed from causes to emotions.


% Concretely, as shown in Figure~\ref{fig:mod_overview}, CDDUDA first performs emotion extraction on the target domain documents using self-training~\cite{chen2011co} based on the knowledge learned from the source domain.
% After obtaining the emotions, CDDUDA simultaneously extracts the causes and emotion-cause pairs of target domain documents in a way of causal disentanglement and discovery through random-editing self-training (introduced in Section \ref{section:cau_par_extraction}).




\subsection{Emotion Extraction}
% \yh{are we still using co-training for our emotion classifier as it performs the best? we use co-training}
% which bridges the gap between source and target domains by gradually adding the most confident predicted target instances from each round to the training set.
\textbf{Document Encoding.} Given a document (either from source or target domain) $d=(c_1,c_2, ..., c_{|d|})$ consisting of $|d|$ clauses, we adopt the first two modules of a hierarchical neural network (as shown in the Step 1 of Figure~\ref{fig:mod_overview}) to generate document-level clause representations.

For each clause $c_i$, we utilize BERT~\cite{devlin2018bert} as a clause encoder to obtain its clause representation $\boldsymbol{c}_i=$BERT$(c_i)\in \mathbb{R}^{d_b}$, where $d_b$ is the output dimension of the pre-trained BERT.
Subsequently, a clause-level bidirectional LSTM~\cite{graves2005framewise} is used to encode $\boldsymbol{c}_i$ into a context-aware clause representation $\boldsymbol{a}_i$:
\begin{equation}
\label{eq:con_awa_cla_representation}
\begin{aligned}
& \overrightarrow{\boldsymbol{a}_i} = \overrightarrow{\text{LSTM}}(\boldsymbol{c}_i, \overrightarrow{\boldsymbol{a}}_{i-1}; \boldsymbol{\theta}_{\text{LSTM}}) \\
& \overleftarrow{\boldsymbol{a}_i} = \overleftarrow{\text{LSTM}}(\boldsymbol{c}_i, \overleftarrow{\boldsymbol{a}}_{i+1}; \boldsymbol{\theta}_{\text{LSTM}}) \\
& \boldsymbol{a}_i = [\overrightarrow{\boldsymbol{a}_i}, \overleftarrow{\boldsymbol{a}_i}] \\
\end{aligned}
\end{equation}
where $\boldsymbol{\theta}_{\text{LSTM}}$ is the parameter of the bidirectional LSTM, $\overrightarrow{\boldsymbol{a}_i}$ and $\overleftarrow{\boldsymbol{a}_i} \in \mathbb{R}^{d_l}$ are respectively the forward and backward hidden states, ${d_l}$ is the hidden size of the bidirectional LSTM, and $\boldsymbol{a}_i$ is the concatenation of $\overrightarrow{\boldsymbol{a}_i}$ and $\overleftarrow{\boldsymbol{a}_i}$.

\textbf{Emotion Extraction.} After getting the contextualized clause representation $\boldsymbol{a}_i$ for each clause, we then feed it into an emotion classifier (the third module of the hierarchical neural network), i.e., softmax regression, to predict the probability of clause $c_i$ being an emotion clause:


\begin{equation}
\label{eq:emo_prediction}
\hat{\boldsymbol{y}}^{e}_{i} = \sigma(\boldsymbol{W}^{\text{sr}}\boldsymbol{a}_{i} + \boldsymbol{b}^{\text{sr}})
\end{equation}
where $\boldsymbol{\theta}_{\text{sr}}=[\boldsymbol{W}^{\text{sr}}; \boldsymbol{b}^{\text{sr}}]$ are the parameters of softmax regression and $\sigma(\cdot)$ is the Softmax function.

Finally, the loss of emotion extraction for a given document $d$ is:
\begin{equation}
\label{eq:emo_loss}
L^{\text{e}}(\boldsymbol{\theta}_{\text{sr}}) = -\sum_{i=1}^{|d|}\boldsymbol{y}^{e}_{i}\log(\hat{\boldsymbol{y}}^{e}_{i})
\end{equation}
where $\boldsymbol{y}^{e}_{i}$ is the emotion annotation of clause $c_i$.


\textbf{Self-training.} Given the loss function in Eq. \ref{eq:emo_loss}, we are now able to use self-training to transfer the knowledge learned from a source domain to a target domain and thus perform cross-domain emotion extraction.
During the training, the hierarchical neural network $h$ maintains a labeled training set $S$ and an unlabeled test set $T$, initialized as $S=\{(d^{s}_{1}, E^{s}_{1}), (d^{s}_{2}, E^{s}_{2}), ..., (d^{s}_{n}, E^{s}_{n}) \}$ and $T=\{(d^{t}_{1}, ?), (d^{t}_{2}, ?), ..., (d^{t}_{n}, ?) \}$ from the source and target domains, respectively. 
$E^{s}_{i}$ denotes the set of emotion annotations of all clauses in a document $d^{s}_{i}$.
In each iteration, $h$ is trained to minimize $L^{e}$ over $S$ then is evaluated on all documents of $T$.
All documents in $T$ that contain predicted emotion clauses above a pre-defined confidence threshold are copied to $S$ for the next iteration.
Each copied document only has one pseudo-labeled emotion clause with the highest probability within the document scope, the remaining clauses are pseudo-labeled as non-emotion ones.
The reason for this is that each document is assumed to have at least one emotion clause and we only consider the strongest one for the ease of training.
% \tw{at least one emotion means one document should have at least one pseudo-labeled emotion clause instead of only one, right?}
Note that if a copied document already exists in $S$, it will be replaced with the latest one (i.e., same document with the latest pseudo-labels) in the current round.
The self-training of $h$ terminates when $S$ does not grow or the emotion clause predictions of all documents in $T$ are below the threshold.






\subsection{Parallel Cause and Emotion-Cause Pair Extraction}
\label{section:cau_par_extraction}
In Step 1, we finally obtain a set of emotions for target domain documents.
Subsequently, we aim to extract the causes of these emotions through causal discovery as it enables us to identify the underlying causal relations given a set of random variables regardless of domain shift.
Once the causes are identified, the corresponding emotion-cause pairs can be naturally derived.
The overall architecture of Step 2 VAE-based causal disentanglement-discovery hierarchical neural network (Vcd hierarchical neural network for short) is shown in the Step 2 of Figure~\ref{fig:mod_overview}.


\subsubsection{Causal Disentanglement for Emotion and Cause Random Variables.}
\label{section:cau_dis_emo_cau_ran_variables}
Since performing causal discovery requires random variables (e.g., emotion and cause variables in a source domain and emotion and event variables \tw{why do we want to mention event variable instead of just using cause here? We did not mention about event variable in the task formulation. Thus I think to keep consistent, it is better to use cause here} in a target domain for our case) and emotion and event (potential cause) variables are mixed in the target domain,
% \tw{a direct reason why disentanglement is needed should be emotion variables are mixed with causal variables instead of only emotion variables are available, right?}
we introduce a causal disentanglement technique that separates out the emotion and cause/event variables in a way of VAE-based DRL.

\textbf{Emotion-cause Pair Encoding.} Given a source domain document $d^{s}$ consisting of emotion-cause pairs $P^{s}=\{(c^{e_1}, c^{c_1}), (c^{e_2}, c^{c_2}), ..., (c^{e_n}, c^{c_n})\}$, for each pair $p_i$, we insert a $[CLS]$ token at the beginning of it and a $[SEP]$ token between its $c^{e_i}$ and $c^{c_i}$, obtaining $(c^{e_i}, c^{c_i})=[CLS] c^{e_i} [SEP] c^{c_i}$. 
Then, we adopt BERT~\cite{devlin2018bert} as a clause pair encoder to obtain each emotion-cause pair representation $\boldsymbol{p}_i=$BERT$((c^{e_i}, c^{c_i}))\in \mathbb{R}^{d_b}$, where $d_b$ is the output dimension of the pre-trained BERT.

For a target domain document $d^{t}=(c_1,c_2, ..., c_{|d|})$ with predicted emotion clauses $E^{t}=(c^{e_1}, c^{e_2}, ..., c^{e_n})$, we first pair each emotion clause $c^{e_i} \in E^{t}$ with all clauses in the document to construct all possible clause pair candidates $P^{t}=\{(c^{e_1}, c_1), (c^{e_1}, c_2), ..., (c^{e_n}, c_{|d|})\}$, where the size of $P^{t}=n*|d|$.
After that, the same clause pair encoding manner as the source domain document is applied.


\textbf{Acquiring Emotion and Cause Random Variables.} After obtaining emotion-cause pair representations $\boldsymbol{p}$ in the source domain,  we utilize two multilayer perceptrons (MLPs) as emotion and cause encoders to learn a set of random variables $\boldsymbol{E}$ and $\boldsymbol{C}$ that respectively represent emotions and causes:
\begin{equation}
\begin{aligned}
\label{eq:emo_cau_encoders}
& \boldsymbol{\mu}^{e}, \boldsymbol{\sigma}^{e} = \text{MLP}(\boldsymbol{p}; \boldsymbol{\theta}_{\text{emo}}) \\
& \boldsymbol{\mu}^{c}, \boldsymbol{\sigma}^{c} = \text{MLP}(\boldsymbol{p}; \boldsymbol{\theta}_{\text{cau}}) \\
& \boldsymbol{E} = \boldsymbol{\mu}^{e} + \boldsymbol{\sigma}^{e}\odot \boldsymbol{\epsilon}, \boldsymbol{\epsilon}\sim\mathcal{N}(\mathbf{0}, \mathbf{I}) \\
& \boldsymbol{C} = \boldsymbol{\mu}^{c} + \boldsymbol{\sigma}^{c}\odot \boldsymbol{\epsilon}, \boldsymbol{\epsilon}\sim\mathcal{N}(\mathbf{0}, \mathbf{I})
\end{aligned}
\end{equation}
where $\boldsymbol{\theta}_{\text{emo}}$ and $\boldsymbol{\theta}_{\text{cau}}$ are respectively the parameters of the emotion and cause encoders, $\boldsymbol{\mu}^{e}$, $\boldsymbol{\sigma}^{e}$ and $\boldsymbol{\mu_}^{c}$, $\boldsymbol{\sigma}^{c}$ are respectively the means and standard deviations of the latent emotion and cause multivariate Gaussian distributions, $\boldsymbol{\epsilon}$ are independent Gaussian noises, $\boldsymbol{E}\in\mathbb{R}^{d_e}$ and $\boldsymbol{C}\in\mathbb{R}^{d_c}$, and $d_e$ and $d_c$ are respectively the number of hidden random variables for emotions and causes.

Since we focus on separating $\boldsymbol{E}$ and $\boldsymbol{C}$ rather than clause pair generation (i.e., the information contained in $\boldsymbol{E}$ and $\boldsymbol{C}$ can decode emotion-cause pairs without considering word order is enough), we adopt the bag-of-words (BoW) features to represent an inputted clause pair and then use them as the predicted target of a clause pair decoder (softmax regression):

\begin{equation}
\label{eq:pair_bow_prediction}
\hat{\boldsymbol{y}}^{p} = \sigma(\boldsymbol{W}^{\text{dec}}[\boldsymbol{e}, \boldsymbol{c}]+ \boldsymbol{b}^{\text{dec}}), \boldsymbol{e}\sim\boldsymbol{E}, \boldsymbol{c}\sim\boldsymbol{C}
\end{equation}
where $\boldsymbol{\theta}_{\text{dec}}=[\boldsymbol{W}^{\text{dec}}; \boldsymbol{b}^{\text{dec}}]$ is the parameters of the decoder, $\boldsymbol{e}$ and $\boldsymbol{c}$ are respectively a sample from $\boldsymbol{E}$ and $\boldsymbol{C}$, $[\cdot, \cdot]$ is concatenation, $\sigma(\cdot)$ is the Softmax function, and $\hat{\boldsymbol{y}}^{p}$ is the predicted pair BoW distribution.

The training objective of the decoder is a cross-entropy loss against the ground-truth pair BoW distribution $y^{p}(\cdot)$:

\begin{equation}
\label{eq:dec_loss}
L^{\text{dec}}(\boldsymbol{\theta}_{\text{dec}}) = -\sum_{\mathclap{w\in \mathcal{W}^{\text{pair}}}}y^{p}(w)\log(\hat{y}^{p}(w))
\end{equation}
where $\mathcal{W}^{\text{pair}}$ is the ground-truth words of a clause pair.

Based on the reconstruction loss Eq. \ref{eq:dec_loss}, the VAE loss is:
\begin{equation}
\label{eq:vae_loss}
\begin{aligned}
L^{\text{VAE}}&(\boldsymbol{\theta}_{\text{emo}}, \boldsymbol{\theta}_{\text{cau}}, \boldsymbol{\theta}_{\text{dec}}) = L^{\text{dec}} +\\ 
& \lambda_{\text{kl}}\text{KL}(q(\boldsymbol{E}, \boldsymbol{C}|\boldsymbol{p})||p(\boldsymbol{E}, \boldsymbol{C}))
\end{aligned}
\end{equation}
where $\lambda_{\text{kl}}$ is a hyperparameter re-weighting the KL term and the reconstruction loss , $p(\boldsymbol{E}, \boldsymbol{C})$ is the prior distribution based on Eq. \ref{eq:emo_cau_encoders}, and $q(\boldsymbol{E}, \boldsymbol{C}|\boldsymbol{p})$ is the posterior distribution regularized by KL-divergence minimization.



To ensure the emotion and cause information is contained in their respective random variables without losing causal relations, we design two auxiliary losses: (1) emotion/cause multi-task loss that ensures $\boldsymbol{E}$/$\boldsymbol{C}$ are discriminative for emotions/causes.
(2) MMD loss that ensures $\boldsymbol{E}$ and $\boldsymbol{C}$ are different but causally related.

With regard to the emotion/cause cross-entropy loss, we build a softmax regression on the random variables $\boldsymbol{E}$ and $\boldsymbol{C}$ respectively to predict the emotion and cause labels:

\begin{equation}
\begin{aligned}
\label{eq:emo_cau_sam_prediction}
& \hat{\boldsymbol{y}}^{\boldsymbol{e}} = \sigma(\boldsymbol{W}^{\text{mul(e)}}\boldsymbol{e} + \boldsymbol{b}^{\text{mul(e)}}), \boldsymbol{e}\sim\boldsymbol{E} \\
& \hat{\boldsymbol{y}}^{\boldsymbol{c}} = \sigma(\boldsymbol{W}^{\text{mul(c)}}\boldsymbol{c} + \boldsymbol{b}^{\text{mul(c)}}), \boldsymbol{c}\sim\boldsymbol{C}
\end{aligned}
\end{equation}
where $\boldsymbol{\theta}_{\text{mul(e)}}=[\boldsymbol{W}^{\text{mul(e)}}; \boldsymbol{b}^{\text{mul(e)}}]$ and $\boldsymbol{\theta}_{\text{mul(c)}}=[\boldsymbol{W}^{\text{mul(c)}}; \boldsymbol{b}^{\text{mul(c)}}]$ are respectively the parameters of the emotion and cause classifiers, $\sigma(\cdot)$ is the Softmax function, and $\hat{\boldsymbol{y}}^{\boldsymbol{e}}$ and $\hat{\boldsymbol{y}}^{\boldsymbol{c}}$ are respectively the predicted emotion and cause distributions.

These two classifiers are trained using the cross-entropy against the ground-truth emotion $y^{e}(\cdot)$ and cause $y^{c}(\cdot)$ distributions: 

\begin{equation}
\label{eq:emo_cau_sam_loss}
\begin{aligned}
& L^{\text{mul(e)}}(\boldsymbol{\theta}_{\text{emo}}; \boldsymbol{\theta}_{\text{mul(e)}}) = -\sum_{\mathclap{l^{e}\in \mathcal{L}^{\text{emo}}}}y^{e}(l^{e})\log(\hat{y}^{e}(l^{e})) \\
& L^{\text{mul(c)}}(\boldsymbol{\theta}_{\text{cau}}; \boldsymbol{\theta}_{\text{mul(c)}}) =-\sum_{\mathclap{l^{c}\in \mathcal{L}^{\text{cau}}}}y^{c}(l^{c})\log(\hat{y}^{c}(l^{c}))
\end{aligned}
\end{equation}
where $\mathcal{L}^{\text{emo}}$ and $\mathcal{L}^{\text{cau}}$ are respectively the ground-truth labels of emotion and cause.
Note that the emotion and cause classifiers are trained along with the emotion and cause encoders, which encourages the entire model not only to predict the emotion and cause of an emotion-cause pair but also to decode its words.
Such the training process can be viewed as multi-task learning \cite{caruana1997multitask} and its loss is denoted by mul($\cdot$).

Regarding the MMD loss, it is imposed for separating $E$ and $C$ from an inputted emotion-cause pair while preserving the causal relation between them, given by:
\begin{equation}
\label{eq:mmd_loss}
\begin{aligned}
L^{\text{mmd}}(\boldsymbol{\theta}_{\text{emo}}, \boldsymbol{\theta}_{\text{cau}}) = -&\Vert\phi(\boldsymbol{e})-\phi(\boldsymbol{c})\Vert^{2}_{\mathcal{H}},\\ &\boldsymbol{e}\sim\boldsymbol{E}, \boldsymbol{c}\sim\boldsymbol{C}
\end{aligned}
\end{equation}
where $\phi$ is a mapping function that projects both $\boldsymbol{e}$ and $\boldsymbol{c}$ into a reproducing kernel Hilbert space denoted by $\mathcal{H}$.
A higher MMD implies $\boldsymbol{E}$ is far away from $\boldsymbol{C}$ or vice versa, that is, the minimization of $L^{\text{mmd}}$ (negative MMD) incentivizes the separation of $\boldsymbol{E}$ and $\boldsymbol{C}$.


\subsubsection{Causal Discovery}
Based on the above causal disentanglement for emotion $\boldsymbol{E}$ and cause $\boldsymbol{C}$ random variables, we are now able to perform causal discovery to identify the causal relations (i.e., edges with directions) between them.
Since the edges naturally point from $\boldsymbol{E}$ to $\boldsymbol{C}$ (i.e., the directions are known if they exist), we introduce a classifier-based causal discovery approach to determine the existence of edges between $\boldsymbol{E}$ and $\boldsymbol{C}$ based on the sample-level dependence of $\boldsymbol{E}$ and $\boldsymbol{C}$.

\textbf{Constructing Positive and Negative Emotion-cause Pairs.} Given a source domain document $d^{s}$ consisting of emotion-cause pairs $P^{s}=\{(c^{e_1}, c^{c_1}), (c^{e_2}, c^{c_2}), ..., (c^{e_n}, c^{c_n})\}$, all pairs in $P^{s}$ are treated as positive samples $S^{P}=\{p_{1}, p_{2}, ..., p_{n}\}$, where $p_{n}=(c^{e_n}, c^{c_n})$.
The construction of negative samples (emotion-non-cause pairs) utilizes each emotion clause in $S^{p}$ to randomly pair any non-cause clause in the document, resulting in the same number of negative samples $S^{N}=\{n_{1}, n_{2}, ..., n_{n}\}$.
Both positive and negative samples are subsequently used to train a causal classifier to discriminate causal and non-causal variables.

\textbf{Discovering Causal Relations between Emotion and Cause Random Variables.} After constructing positive and negative samples, we first feed them into the clause pair encoder then pass to the emotion and cause encoders to obtain a set of emotion $\boldsymbol{E}$ and event $\boldsymbol{V}$ random variables.
Here, we have event variables instead of cause ones as we mix cause and non-cause clauses from the positive and negative samples.
To discover causal relations between $\boldsymbol{E}$ and $\boldsymbol{V}$, we build a sample-level causal classifier, given by:
\begin{equation}
\label{eq:pair_causal_prediction}
\hat{\boldsymbol{y}}^{v} = \sigma(\boldsymbol{W}^{\text{mul(v)}}[\boldsymbol{e}, \boldsymbol{v}]+ \boldsymbol{b}^{\text{mul(v)}}), \boldsymbol{e}\sim\boldsymbol{E}, \boldsymbol{v}\sim\boldsymbol{V}
\end{equation}
where $\boldsymbol{\theta}_{\text{v}}=[\boldsymbol{W}^{\text{mul(v)}}; \boldsymbol{b}^{\text{mul(v)}}]$ is the parameters of the causal classifier, $\boldsymbol{e}$ and $\boldsymbol{v}$ are respectively a sample from $\boldsymbol{E}$ and $\boldsymbol{V}$, $[\cdot, \cdot]$ is concatenation, $\sigma(\cdot)$ is the Sigmoid function, and $\hat{\boldsymbol{y}}^{v}$ is the predicted Bernoulli distribution indicating whether $\boldsymbol{e}$ and $\boldsymbol{v}$ have a causal relation.
The intuition here is that if $\boldsymbol{v} \rightarrow \boldsymbol{e}$, then $\boldsymbol{v} \perp \boldsymbol{e}$ must exist, i.e., the dependence between $\boldsymbol{v}$ and $\boldsymbol{e}$ predicted by the causal classifier implies the underlying causal relation.

The training of the causal classifier is to minimize the cross entropy between $\hat{\boldsymbol{y}}^{v}$ and the ground-truth distribution $y^{v}(\cdot)$:
\begin{equation}
L^{\text{mul(v)}}(\boldsymbol{\theta}_{\text{emo}},\boldsymbol{\theta}_{\text{cau}}; \boldsymbol{\theta}_{\text{mul(v)}}) =-\sum_{\mathclap{l\in \mathcal{L}^{\text{causal}}}}y^{v}(l)\log(\hat{y}^{v}(l))
\end{equation}
where $\mathcal{L}^{\text{causal}}$ is the ground-
truth labels of positive and negative samples, with 1 and 0 indicating that their emotion and event clause pairs have causal and non-causal relations, respectively.
Similar to the losses in Eq. \ref{eq:emo_cau_sam_loss}, the training of causal classifier is also multi-task learning, which facilitates the entire model to distinguish causal and non-causal variables.

Finally, we employ the sum of all the losses depicted in Section \ref{section:cau_par_extraction} as the overall loss of Step 2 Vcd hierarchical neural network:
\begin{equation}
\label{eq:ove_loss}
\begin{aligned}
L^{\text{Vcd}}&=L^{\text{VAE}}(\boldsymbol{\theta}_{\text{emo}}, \boldsymbol{\theta}_{\text{cau}}, \boldsymbol{\theta}_{\text{dec}})\\ &+\lambda_{\text{mul(e)}}L^{\text{mul(e)}}(\boldsymbol{\theta}_{\text{emo}}; \boldsymbol{\theta}_{\text{mul(e)}})\\
&+\lambda_{\text{mul(c)}}L^{\text{mul(c)}}(\boldsymbol{\theta}_{\text{cau}}; \boldsymbol{\theta}_{\text{mul(c)}})\\
&+\lambda_{\text{mmd}}L^{\text{mmd}}(\boldsymbol{\theta}_{\text{emo}}, \boldsymbol{\theta}_{\text{cau}})\\
&+\lambda_{\text{mul(v)}}L^{\text{mul(v)}}(\boldsymbol{\theta}_{\text{emo}},\boldsymbol{\theta}_{\text{cau}}; \boldsymbol{\theta}_{\text{mul(v)}})
\end{aligned}
\end{equation}
where $\lambda$s are the hyperparameters balancing the above losses. 


\subsubsection{Random-editing Self-training}
Given the loss function in Eq. \ref{eq:ove_loss}, we aim to transfer the causal knowledge obtained from a source domain to a target domain, enabling cross-domain emotion-cause pair extraction. 
To do that, we introduce a random-editing self-training approach that allows a source-trained model to adapt the causal knowledge to a target domain without memorization.

First, the Vcd hierarchical neural network $h^{\text{Vcd}}$ is trained on the constructed source domain data consisting of both positive and negative samples (pairs), denoted by $O=\{(d^{s}_{1}, P^{s}_{1}), (d^{s}_{2}, P^{s}_{2}), ..., (d^{s}_{n}, P^{s}_{n}) \}$.
$P^{s}_{i}$ denotes the set of positive and negative emotion-cause pair annotations in a document $d^{s}_{i}$.
Then, in each iteration, $h^{\text{Vcd}}$ is trained to minimize $L^{\text{Vcd}}$ over the the target domain data $A=\{(d^{t}_{1}, \hat{P}^{t}_{1}), (d^{t}_{2}, \hat{P}^{t}_{2}), ..., (d^{t}_{n}, \hat{P}^{t}_{n}) \}$, where $\hat{P}^{t}_{i}$ denotes the set of positive and negative pseudo-labeled  emotion-cause pairs predicted in the previous round for a document $d^{t}_{i}$.
Note that, before the start of training, all possible pair candidates in a target domain document are obtained based on its predicted emotion clauses (see Section \ref{section:cau_dis_emo_cau_ran_variables}).
In the construction of pseudo-labeled pairs, we select a pair with the highest probability within the document scope as a positive sample and randomly choose a pair from the remaining pairs as a negative sample.
Such the mechanism can help a model to avoid memorizing noisy samples in the early stage of training.
The random-editing self-training of $h^{\text{Vcd}}$ terminates when a pre-defined iteration number is reached.



% $h^{\text{Vcd}}$ is used to generate positive and negative pseudo-labeled samples on . 







==> prel.tex <==
\section{Problem Analysis from a Causal View}
\label{sec:problem_analysis}
We investigate the \task task and its challenges from a causal perspective.
\paragraph{Preliminaries on Causal Discovery.}
\label{sec:preliminaries_cd}
Given $N$ random variables $ \{X_n\}^N_{n=1} $, causal discovery aims to identify the causal relations among them~\cite{guo2020survey}. If there is a causal relation from $X_m$ to $X_n$, denoted by an edge between them $X_m \rightarrow X_n$, manipulating $X_m$ changes $X_n$. A causal graph consists of a set of such relations~\cite{pearl2000causality}, forming the structures, such as chain, immorality and fork, as shown in Figure~\ref{fig: cau_discovery}.

\begin{figure}[hbt!]
    \centering
    \includegraphics[width=\linewidth]{figures/cau_discovery.png}
    \caption{An example of causal discovery.}
    \label{fig: cau_discovery}
\end{figure}


Causal discovery from purely observational data has been well studied~\cite{glymour2019review,guo2020survey}.
For ease, we consider the problem of recovering a graph $G$ with three nodes $X$, $Y$ and $Z$ from the data sampled from a joint probability distribution $P$. By applying the methods, e.g. statistical tests, we can identify the (conditional) independencies between random variables. The majority of the causal discovery algorithms make the \textit{faithfulness assumption} that we can infer the d-separation structure of a graph from independencies in a distribution~\cite{pearl2000causality}. 
%To recover the underlying causal structure in $G$, we need to infer d-separations in $G$ from conditional independencies in $P$, which is supported by the faithfulness assumption:
\begin{equation}
    X \indep_{G} Y | Z \leftarrow X \indep_{P} Y | Z
\end{equation}
where $X \indep_{G} Y | Z$ denotes $X$ is d-separated with $Y$ in $G$ conditioned on $Z$ and $X \indep_{P} Y | Z$ denotes $X$ is independent with $Y$ in $P$ conditioned on $Z$.

Constraint-based approaches are a family of algorithms commonly used for causal discovery.
The PC algorithm~\cite{spirtes2000causation} is a  typical example in this family.
It begins with adding an undirected edge between a pair of random variables if a statistical independence test finds out that they are dependent, then recursively removes edges if a pair of variables are found to be independent conditioned on a set of other variables. Hence, the discovery process is exponential to the number of variables. Finally, the algorithm finds orientation of edges by apply search heuristics and making use of the statistical properties of the immorality structure.
%Specifically, the skeleton of the graph (i.e., the true undirected \tw{should be directed, right?} graph) is first identified by gradually increasing conditioning sets.
%Subsequently, the immorality structure within the skeleton is identified as its property is distinct from the chain and fork structures (e.g., in Figure~\ref{fig: cau_discovery}, the association between $X_1$ and $X_3$ in an immorality is unblocked by conditioning on $X_5$).
%Finally, the remaining edges are oriented as much as possible based on previously discovered immoralities.
%This is due to the indistinguishability between chain and fork (i.e., they could share the same set of independencies).

\begin{figure*}[hbt!]
     \centering
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/ama_domains1.png}
         \caption{Amazon sentiment reviews}
         \label{fig: amazon}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/ch_emotion.png}
         \caption{Chinese emotion clauses}
         \label{fig: chi_emotion}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/ch_cause.png}
         \caption{Chinese emotion cause clauses}
         \label{fig: chi_cause}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/en_emotion.png}
         \caption{English emotion clauses}
         \label{fig: en_emo}
     \end{subfigure}
     \begin{subfigure}[b]{0.31\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/en_cause.png}
         \caption{English emotion cause clauses}
         \label{fig: en_emo}
     \end{subfigure}
     \caption{The t-SNE visualizations of the sentence embeddings from Amazon Reviews multi-domain sentiment corpus, the clause embeddings from the Chinese and English \task corpora.}
     \label{fig:CD-ECPE_challenges}
\end{figure*}

\paragraph{A Causal View of the Task.}
\label{sec:causal_view}
All prior studies on the \targettask task and the identification of causal relations~\cite{moghimifar2020learning} employ a (deep) learning-based classifier to detect causal relations in text. As those classifiers make decisions purely based on associations, it seems to contradict to the well-known statement in the causality theory that `Correlation is not causation.''. From the last section, we know that causal structures, at least parts of them, can be inferred from independence test results. One family of such statistical tests are to build a classifier to determine if two random variables are dependent or not based on a sample of data~\cite{lopez2016revisiting}. Herein, the classifier is trained by a set of data annotated with binary labels, which is 1 if a pair of data points is dependent and 0 otherwise. Then its predictions on a new sample are used to calculate the statistics for the test results. Hence, the prior NLP models for the target task can be viewed as taking the first step of the PC algorithm that infers causal relations by estimating the dependence between the underlying random variables given an input text. Herein, they make an implicit assumption that if the random variable of an event and the random variable of an emotion are statistically dependent, then the event is a direct cause of that emotion.
%In this section, we identify the assumptions made by the prior works on \targettask and investigate its connections to causal discovery. According to the causality theory~\cite{neal2020causalitybook}, ``Correlation is not causation.'' such that we cannot simply conclude one event causes the other just because two events correlate. Two random variables may be correlated through a cofounder that influences both of them. For example, in Fig.\ref{fig: cau_discovery}, $X_1$ and $X_3$ becomes dependent through $X_2$ in the chain and fork structures although there is no direct causal relation between them. For \targettask, we are interested in if an event is a direct cause to an emotion, which can be interpreted as checking if there is an edge between two corresponding latent random variable vectors, but we do not want to recover complete causal graphs from observational data. Inspired by constrained-based causal discovery algorithms and the faithfulness assumption, the problem is reduced to applying statistical tests to infer causal relations based on their dependence structures. 

%Constrained-based causal discovery algorithms are computationally expensive, thus we adopt an assumption used in all prior works~\cite{xia2019emotion} that if the random variable vector of an event and the random variable vector of an emotion are statistically dependent, then the event is a direct cause of that emotion. Removing that assumption requires curation of new corpora and design of computationally more efficient algorithms, which is beyond the scope of this work. 
In this work, we also make the same assumption. Thus, we investigate to what degree the assumption holds in the existing datasets. As causes are usually mentioned before effects in a document, we find out that in the Chinese \targettask corpus (\checpe)~\cite{xia2019emotion}, 89.24\% of the annotated event mentions occur before or within the clause of the corresponding emotional expression, and the ratio is 80.01\% in the English \targettask corpus (\enecpe)~\cite{singh2021end}. We conjecture that it might be the reason why the orientation of relations is not an issue in such corpora. Based on the theory, it is clear that the existing approaches omit the influence of cofounders. As there are a large number of distinct events in a corpus, which require an exponential number of conditional independence tests, thus we leave this problem for future work. %As statistical models are purely based on associations, if such models are directly applied to causal relation extraction without any assumptions, the corresponding predictions are not reliable. 

%After manually inspecting the current emotion-cause pair dataset \thuctc, we find that almost all the emotion-cause pairs satisfy the assumption that an event causes an emotion if an event statistically depends on an emotion type at the semantic level.\lqu{Yujin, you may need to check how to support the assumption. There might be another condition that if an emotional expression occurs after the mention of the event.} \yh{Chinese: 89.24\% (cause before and equal emotion), English: 80.01\% (cause before and equal emotion)} It is a stronger assumption than the faithfulness assumption but widely used in the prior works~\cite{xia2019emotion}, though it is not explicitly mentioned.

%To characterize events and emotions in the semantic space, we assume their latent representations carry the meanings and form a sample space. This assumption is inspired by the common practice that hidden representations of deep neural networks are used for semantic analysis~\cite{}. In particular, we introduce a random variable vector $\vz^x$ for each event $x$ and a random variable vector $\vz^e$ for each emotion $e$, where an emotion is a fine-grained representation of a mental state and can be assigned to a category $y \in \gY$. If $\vz^x \dep \vz^e$, then $\vz^x \rightarrow \vz^e$ according to our assumption.

%Another challenge is that we only observe mentions of events and emotional expressions. Hence, we need to learn a projection function from the space $\gX$ to the latent space $\gZ$ before applying any statistical tests. Such a function can be realized as an encoder, the marginal probability $p(\rmX) = \int p(\rmX | \vz_0, ..., \vz_d)p(\vz_0, ..., \vz_d)d\vz$ of data is intractable. Hence we employ the variational autoencoder (VAE) techniques~\cite{}.

%Due to the need of carrying out dependence tests on latent representations, we adapt the classifier-based dependence test~\cite{} to our problem. This classifier-based test utilizes a classifier to determine if a pair of random variables are dependent or not. As we are concerned with if an emotional expression is the result of an event mentioned in the same document, we use the classifier directly to infer if their corresponding random variables are dependent or not, given a latent emotion representation and a latent event representation, generated by the VAE model.


\paragraph{Challenges in UDA.}
To have an intuitive understanding of the challenges in the UDA setting, we visualize the clause embeddings for ground-truth emotion and emotion causes respectively on \checpe and \enecpe, and compare them with the sentence embeddings for a widely used domain adaptation corpus Amazon Reviews~\cite{blitzer2007biographies} using t-SNE.
The details about dividing those \targettask corpora into domains are provided in Sec. \ref{exp_setup}.
\dv{As shown in Figure~\ref{fig:CD-ECPE_challenges}, these data points from various \checpe's domains are mixed and scattered throughout the entire region, making them much more challenging to be distinguished comparable to the sentence embeddings in the Amazon corpus.
In contrast, to validate the model's domain adaption ability, we employ two different datasets within the context of the English language.
Therefore, in Figure~\ref{fig:CD-ECPE_challenges} (d) and (e), it can be noted that though some of the samples are overlapping with each other, there is a very clear boundary between the two domains.}
It is thus challenging for existing UDA methods, which work only in the cases that the distribution shift from a source domain to a target domain is small~\cite{zhao2019learning,kumar2020understanding}.






==> tab_corpus_statistics.tex <==
\begin{table*}[hbt!]
\centering
\small
\begin{tabular}{cccccc} 
\noalign{\hrule height 1.8pt}
Language                 & Domain        & Docs. with 1 pair & Docs. with 2 pairs & Docs. with > 2 pairs & All  \\ 
\hline
\multirow{5}{*}{Chinese} & Society (S)       & 1045 & 99 & 17 & 1161 \\
                         & Entertainment (T) & 111 & 8 & 0 & 119     \\
                         & Home (T)          & 96 & 13 & 3 & 112     \\
                         & Education (T)     & 121 & 9 & 0 & 130     \\
                         & Finance (T)       & 79 & 10 & 1 & 90      \\ 
\hline
\multirow{5}{*}{English} & History (S)   & 712 & 99 & 20 & 831 \\
                         & War (T)       & 121 & 5  & 0  & 126 \\
                         & Romance (T)   & 161 & 14 & 0  & 175 \\
                         & Adventure (T) & 112 & 12 & 3  & 127 \\
                         & Biography (T) & 90  & 5  & 0  & 95  \\
\noalign{\hrule height 1.8pt}
\end{tabular}
\caption{The statistics of the CD-ECPE corpus. “Docs.”, "S" and "T" are the abbreviations for “Documents”, "Source domain" and "Target domain", respectively.}
\label{table: corpus_stat}
\end{table*}
